Preference-based Pure Exploration

We study the preference-based pure exploration problem for bandits with vector-valued rewards. The rewards are ordered using a (given) preference cone $\mathcal{C}$ and our goal is to identify the set of Pareto optimal arms. First, to quantify the impact of preferences, we derive a novel lower bound on sample complexity for identifying the most preferred policy with a confidence level $1-\delta$. Our lower bound elicits the role played by the geometry of the preference cone and punctuates the difference in hardness compared to existing best-arm identification variants of the problem. We further explicate this geometry when the rewards follow Gaussian distributions. We then provide a convex relaxation of the lower bound and leverage it to design the Preference-based Track and Stop (PreTS) algorithm that identifies the most preferred policy. Finally, we show that the sample complexity of PreTS is asymptotically tight by deriving a new concentration inequality for vector-valued rewards.

==> paper/numerical-experiment.tex <==
We evaluate the performance of Adaptive Pareto Exploration on a real-world scenario and on synthetic random by benchmarking the performance with AdapPareto in~\cite{kone2023adaptive} and a naive adaptation of~\cite{auer2016pareto}. 



\subsection{Synthetic Dataset}
To further illustrate the impact of in comparison with PSI-Unif-Elim by using 2000 randomly generated multi-variate Gaussian instances, with $K = 5$ arms and different values of the dimension $\numobj$. We set $\delta = 0.1$.

\subsection{Realworld Dataset}
We use SNW dataset from~\cite{zuluaga2013active} and  for linear bandits. It consists of $206$ different hardware implementations of a sorting network. The objectives are the area and throughput of the network when synthesized on an FPGA $L=2$. Since we consider maximization problems, we use the negative of area as objective value. The mean rewards of designs are taken as the objective values in the dataset. The reward vector of a design is formed by adding independent zero mean Gaussian noise with variance $\sigma^{2}=1$ to the mean value of each objective of the design.




==> paper/technical_lemma.tex <==
\newpage
\section{Technical Lemmas}
\begin{lemma}\label{lem:ind-concentration}
For any $k=1,2,\ldots,K$, let $1 \le t_{k} \le t$. Let $\eta >0$ and define the event: 
\[
C \triangleq \cap_{k \in [K]} C_{k} \triangleq \cap_{k \in [K]} \{t_k \le N_{k,t} \le (1+\eta) t_k\}
\] and let $\mathbbm{1}_{C}$ indicate whether the event holds. For $\rho \ge (1+\eta)K$, for all $z \in \cone$ we have:
\[
\mP\left[\ind{C}\sum_{k \in [K]} \numarmkt \klobjl \ge \rho \right] \le \left(\frac{\rho e}{K}\right)^{K}\exp\left(\frac{-\rho}{1+\eta}\right)\,.
\]
\end{lemma}
\begin{proof}
Fix $\zeta \in \mR^{K}_{+}$ and $t \ge 0$. Define $m_{k,t}$ such that:
\begin{eqnarray*}
m_{k,t} &=& 
\begin{cases}
m, \ \text{if} \ \exists \ 0 \le m \le z^{\top}M_{k}, \ \text{s.t.} \ t \kl{m}{z^{\top}M_{k}} = \zeta_{k} \\
0, \ \text{otherwise}
\end{cases}
\end{eqnarray*}
By monotonicity of $t\kl{}{}, \ t \rightarrow m_{k,t}$ is increasing. With $t=N_{k,t}$, we have that 
\[
N_{k,t}\kl{m_{k,N_{k,t}}}{z^{\top} M_{k}} = \zeta_{k} \le N_{k,t}\kl{z^{\top}\mklestm}{z^{\top}M_{k}}, \implies z^{\top} \mklestm \stackrel{(a)}{\le} m_{k,N_{k,t}} \stackrel{(b)}{\le} m_{k,(1+\eta)t_k},
\] 
where $(a)$ follows from monotonicity of $\kl{\cdot}{\cdot}$ and $(b)$ follows from monotonicity of $m^{(\ell)}_{k,t}$. 

With $t_k \kl{z^{\top}\hat{M}_{k,t_k(1+\eta)}}{z^{\top}M_{k}} = \frac{\zeta_{k}}{1+\eta}$ and non-negativity of $\kl{\cdot}{\cdot}$ we have:
\begin{eqnarray*}
&\quad& \mP\left( \cap_{k \in [K]}\left\{\mathbbm{1}_{C_k} N_{k,t} \klobjl \ge \zeta_{k}\right\} \right)\\
&\le& \mP\left( \cap_{k \in [K]} \left\{ z^{\top}\mklestm \le m_{k,N_{k,t}}, C_{k}\right\} \right) \\
&\le& \mP\left( \cap_{k \in [K]} \left\{ z^{\top}\mklestm \le m_{k,(1+\eta)t_{k}}, C_{k}\right\} \right) \\
&\le& \mP\left(\cap_{k \in [K]} \left\{ z^{\top}\mklestm \le m_{k,(1+\eta)t_{k}} , C_{k}\right\} \right) \\
&\stackrel{(a)}{\le}& \exp\left(-\sum_{k \in [K]}t_{k}\kl{m_{k,(1+\eta)t_{k}}}{z^{\top}M_{k}}\right)\\
&=& \exp\left(-\sum_{k \in [K]}\frac{\zeta_k}{1+\eta}\right)\,,
\end{eqnarray*}
where $(a)$ follows from Lemma~\ref{lem:kl-exp-bound}. 

Using Lemma~\ref{lem:multidim-exp-sum}, with $Z_{k} = \numarmkt \klobjl$ and $a = \frac{1}{(1+\eta)}$, we have that:
\[
\mP\left[\ind{C}\sum_{k \in [K]}\numarmkt \klobjl \ge \rho \right] \le \left(\frac{\rho e}{K}\right)^{K}\exp\left(\frac{-\rho}{1+\eta}\right)
\]
This concludes the proof.
\end{proof}
\iffalse
Alternative proof:
\begin{proof}
Fix $\zeta \in \mR^{K}_{+}$ and $t \ge 0$. Define $m^{(\ell)}_{k,t}$ such that:
\begin{eqnarray*}
m^{(\ell)}_{k,t} &=& 
\begin{cases}
m, \ \text{if} \ \exists \ 0 \le m \le M^{(\ell)}_{k}, \ \text{s.t.} \ t \kl{m}{M^{(\ell)}_{k}} = \zeta^{(\ell)}_{k} \\
0, \ \text{otherwise}
\end{cases}
\end{eqnarray*}
By monotonicity of $t\kl{}{}, \ t \rightarrow m^{(\ell)}_{k,t}$ is increasing. With $t=N_{k,t}$, we have that 
\[
N_{k,t}\kl{m^{(\ell)}_{k,N_{k,t}}}{M^{(\ell)}_{k}} = \zeta^{(\ell)}_{k} \le N_{k,t}\kl{\mklestm}{\mkl}, \implies \mklestm \stackrel{(a)}{\le} m^{(\ell)}_{k,N_{k,t}} \stackrel{(b)}{\le} m^{(\ell)}_{k,(1+\eta)t_k},
\] 
where $(a)$ follows from monotonicity of $\kl{\cdot}{\cdot}$ and $(b)$ follows from monotonicity of $m^{(\ell)}_{k,t}$. 

With $t_k \kl{z^{\top}\hat{M}_{k,t_k(1+\eta)}}{z^{\top}M^{(\ell)}_{k}} = \frac{\zeta_{k}}{1+\eta}$ and non-negativity of $\kl{\cdot}{\cdot}$ we have:
\begin{eqnarray*}
&\quad& \mP\left( \cap_{k \in [K]}\left\{\mathbbm{1}_{C_k} N_{k,t} \klobjl \ge \sum_{\ell} \zeta_{k,\ell}\right\} \right)\\
&\le& \mP\left( \cap_{k \in [K]}\left\{\mathbbm{1}_{C_k}  N_{k,t} \sum_{\ell} z^{\ell} \kl{\hat{M}^{(\ell)}_{k,t}}{M_{k,\ell}} \ge \sum_{\ell} \zeta_{k,\ell}\right\} \right)\\
&\le& \mP\left( \cap_{k \in [K]} \left\{ \mklestm \le m^{(\ell)}_{k,N_{k,t}}, C_{k}\right\} \right) \\
&\le& \mP\left( \cap_{k \in [K]} \left\{ \mklestm \le m^{(\ell)}_{k,(1+\eta)t_{k}}, C_{k}\right\} \right) \\
&\le& \Pi_{k \in [K]}\mP\left( \left\{ \mklestm \le m^{(\ell)}_{k,(1+\eta)t_{k}} , C_{k}\right\} \right) \\
&\stackrel{(c)}{\le}& \Pi_{k \in [K]} \exp\left( -(1+\eta)t_{k}\kl{M^{(\ell)}_{k}}{m^{(\ell)}_{k}(t)}\right) \\
&=& \exp\left(-\sum_{k \in [K]}(1+\eta)t_{k}\kl{M^{(\ell)}_{k}}{m^{(\ell)}_{k}(t)}\right)
\end{eqnarray*}
where, the $(c)$ follows from Lemma~\ref{lem:kl-exp-bound}. Using Lemma~\ref{lem:multidim-exp-sum}, with $Z_{k,\ell} = \numarmkt \klobjl$ and $a = \frac{1}{(1+\eta)}$, we have that:
\[
\mP\left[\ind{C}\sum_{k \in [K]}\numarmkt \klobjl \ge \rho \right] \le \left(\frac{\rho e}{K}\right)^{K}\exp\left(\frac{-\rho}{1+\eta}\right)
\]
This concludes the proof.
\end{proof}
\fi

\begin{lemma}
\label{lem:kl-exp-bound}
For any $k=1,2,\ldots,K$ let $1\le t_k \le t$. Then for all $0 \le C_{k} \le M^{(\ell)}_{k}$ we have 
\[
\mP\left(\cap_{k \in [K]} \cap_{\ell \in [L]} \left\{ z^{\top}\hat{M}_{k,t} \le C_{k},\ t_{k} \le N_{k,t}\right\} \right) \le \exp\left( -\sum_{k \in [K]}\sum_{\ell \in [L]} t_k\klobjl\right)\,.
\]
\end{lemma}
\begin{proof}
For all $k \in [K]$ define the moment generating function as:
\[
\phi^{(\ell)}_{k}(\lambda) = \ln \mE_{M^{(\ell)}_{k}}\left[ \exp(\lambda X) \right],
\] 
where $X$ is sampled from a single-parameter exponential family with mean $M^{(\ell)}_{k}$. From Donsker-Vardhan Variational Formula, (Theorem~\ref{thm:donsker-vardhan} in Appendix~\ref{sec:aux}), we have that: 
\[
\kl{M^{(\ell)}_{k}}{\hat{M}^{(\ell)}_{k,t}} =  \sup_{\lambda \le 0} \mE_{\hat{M}^{(\ell)}_{k,t}} \left[ \lambda X\right] - \ln \mE_{M^{(\ell)}_{k}} \left[ \exp(\lambda X) \right]
\]


Define the events $\cE_{1}:= \cap_{k \in \armset} \left\{t_k \le  N_{k,t}\right\}$ and $\cE_{2}:= \cap_{k \in \armset}\cap_{\ell \in [L]} \left\{ \hat{M}^{(\ell)}_{k,t} \le C^{(\ell)}_{k}\right\}$ and $\cE = \cE_{1} \cap \cE_{2}$.

\medskip 
Define the martingale $G_t = \exp\left( \sum_{k \in [K]} \sum_{\ell \in [L]} \lambda^{(\ell)}_{k} X_{k,t} - N_{k,t} \phi^{(\ell)}_{k}(\lambda^{(\ell)}_{k})\right)$. For all $t' \le t, \ G_{t'} = G_{t'-1}\exp\left(\sum_{k \in [K]} \sum_{\ell \in [L]} \lambda^{(\ell)}_{k} X_{k,t'} - N_{k,t'} \phi^{(\ell)}_{k}(\lambda^{(\ell)}_{k})\right) $ 
We deduce $\mE \left[ G_{t'} \vert \cF_{t'-1} \right] = G_{t'-1}$ and $\mE\left[G_{t}\right] = 1$. 

\medskip 
We then define 
\begin{eqnarray*}
\mP\left(\cE\right) &=& \mP\left( \cap_{k \in [K]} \cap_{\ell \in [L]} \left\{ X_{k,t} \le N_{k,t} C^{(\ell)}_{k} \right\} \wedge \cE_{1}\right) \\ 
&\le&  \mP\left( \ind{\cE_{1}} \times \mathbbm{1}\left\{\sum_{k \in [K]}\sum_{\ell \in [L]} \lambda^{(\ell)}_{k} X_{k,t} \ge \sum_{k \in [K]}\sum_{\ell \in [L]} \lambda^{(\ell)}_{k} N_{k,t} C^{(\ell)}_{k}\right\} \right)\\
&\le& \mP\left(\ind{\cE_{1}}\times \mathbbm{1}\left\{\exp\left(\sum_{k \in [K]}\sum_{\ell \in [L]} \lambda^{(\ell)}_{k} X_{k,t} \right)  \ge \exp\left(\sum_{k \in [K]}\sum_{\ell \in [L]} \lambda^{(\ell)}_{k} N_{k,t} C^{(\ell)}_{k} \right)\right\}\right) \\
&\le& \mP\left(\ind{\cE_{1}}\times \mathbbm{1}\left\{ G_t \ge \exp\left(\sum_{k \in [K]}\sum_{\ell \in [L]} \lambda^{(\ell)}_{k} N_{k,t} C^{(\ell)}_{k} - \lambda^{(\ell)}_{k}\phi^{\ell}_{k}\right)\right\}\right) \\
&\le& \mP\left(\ind{\cE_{1}} \times \mathbbm{1}\left\{G_t \ge \exp\left(\sum_{k \in [K]}\sum_{\ell \in [L]} N_{k,t} (\lambda^{(\ell)}_{k}C^{(\ell)}_{k} - \phi^{\ell}_{k}) \right)\right\}\right) \\
&\le& \mP\left(\ind{\cE_{1}}\times \mathbbm{1}\left\{G_t \ge \exp\left(\sum_{k \in [K]}\sum_{\ell \in [L]} N_{k,t}\kl{M^{(\ell)}_{k}}{(m^{(\ell)}_{k,t}}\right)\right\}\right) 
\end{eqnarray*}
Using Markov's inequality and $\mE\left[G_t\right]=1$, we have:
\begin{align*}
\mP\left[\cE\right] &= \mE\left[\ind{\cE_1} G_t \right] \exp\left( -\sum_{k \in [K]} \sum_{\ell \in [L]} N_{k,t} \kl{M^{\ell}_{k}}{m^{(\ell)}_{k}} \right)\\
&\le \exp\left( -\sum_{k \in [K]} \sum_{\ell \in [L]} N_{k,t} \kl{M^{\ell}_{k}}{m^{(\ell)}_{k}} \right)    
\end{align*}
\end{proof}


\begin{lemma}
\label{lem:multidim-exp-sum}
Let $a > 0$ and $K \ge 2$ and $Z \in \mR^{K \times L}$ such that for all $\xi \in \mR^{K \times L}_{+}$ we have:
\[
\mP\left( Z  \ge  \zeta \right) \le \exp\left(-a\sum_{k \in [K]} \sum_{\ell \in [L]} \zeta^{(\ell)}_{k} \right)
\]
Then, for all $\rho \ge \frac{KL}{a} \in \mR_{+}$ , we have:
\[
\mP\left( \sum_{k \in [K]} \sum_{\ell \in [L]} Z_{k,\ell} \ge  \rho\right) \le \left(\frac{ae\rho}{KL}\right)^{KL} \exp(-a\rho)
\]
\end{lemma}

\begin{proof}
Let $Y_k \in \mR^{KL}$ be a vector whose components are drawn independently from an exponential distribution with mean $a$. Then, using Lemma~\ref{lem:peskun-order} for all $\eta \in \mR^{KL}$, we have that: 
\[
\mP\left(Z \ge \eta \right) \le_{s} \exp\left(-a\sum_{k}\sum_{\ell} \eta_{k\ell} \right) = \mP\left(Y  \ge \eta \right)
\]
For $\lambda \in [0,a), \ \rho \in \mR^{+}$ using Markov's inequality: 
\begin{eqnarray*}
\mP\bigg[\sum_{k}\sum_{\ell} Z_{k,\ell} \ge \rho\bigg] &=& \mP\bigg[\exp\left(\lambda \sum_{k}\sum_{\ell} Z_{k\ell} \ge \exp(\lambda \rho) \right)\bigg]\\
&\le& \exp\left(-\lambda \rho \right) \mE\left[\exp\left(\lambda \sum_{k}\sum_{\ell} Z_{k,\ell} \right)\right]\\
&\le& \exp\left(-\lambda \rho\right)\mE\left(\Pi_{k}\Pi_{\ell} \exp(\lambda Z_{k\ell})\right) \\
&\le& \exp\left(-\lambda \rho\right) \mE\left[\Pi_{k}\Pi_{\ell
} \exp\left(\lambda Y_{k\ell}\right)\right] \\
&=& \exp\left(-\lambda \rho\right) \Pi_{k} \Pi_{\ell} \mE\left[\exp\left(\lambda Y_{k \ell}\right)\right]
\end{eqnarray*}
Since, $Y_{k\ell}$ follow an exponential distribution, we have $\mE\left[\exp(\lambda Y_{k\ell})\right]=\int_{0}^{\infty} a \exp(-ay) \exp(a\lambda)dy = \frac{a}{a-\lambda}$.  We have for all $0 \le \lambda < a$: 
\[
\mP\left[ \sum_{k}\sum_{\ell} Z_{k\ell} \ge \rho \right] \le \exp(-\lambda \rho) \frac{a^{KL}}{(a-\lambda)^{KL}}
\] 
Setting $\lambda = a- \frac{KL}{\rho}$, we get the result.
\end{proof}


